Measuring Monosemanticity in Sparse Autoencoders via Latent Activation Coherence

Within Explainable Artificial Intelligence, mechanistic interpretability uses Sparse Autoencoders (SAEs) to extract more interpretable features from neural representations. However, assessing their monosemanticity, and thus explanation quality, remains challenging. Existing metrics require external concept labels or depend on pretrained embedding models, making them sensitive to encoder's geometry. We introduce the Tversky Monosemanticity Score (TMS), a label-free metric that operationalizes monosemanticity as activation-set coherence of binarized SAE latents, and does not require external embedding encoders. We evaluate TMS on SAEs trained on features from pretrained vision and vision-language models (DINOv3, CLIP, BLIP2), two common SAE regimes (TopK, BatchTopK), multiple sparsity levels, and expansion factors. Our results show that TMS is less affected by encoder anisotropy than its embedding-based alternative, while remaining aligned with established monosemanticity indicators. TMS also reveals distinct SAE training dynamics across base models. Moreover, under encoder anisotropy, TMS provides a stronger indication of probe-based concept deletion effectiveness, while being competitive otherwise.

==> FIGS/corr/blip/nontarget_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Non-target drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]
            
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.0017)
              (2,  0.0045)
              (4,  0.0077)
              (8,  0.0109)
              (16, 0.0147)
              (32, 0.0179)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.0047)
              (2,  0.0109)
              (4,  0.0250)
              (8,  0.0410)
              (16, 0.0547)
              (32, 0.0708)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.0009)
              (2,  0.0022)
              (4,  0.0044)
              (8,  0.0076)
              (16, 0.0094)
              (32, 0.0117)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.0032)
              (2,  0.0085)
              (4,  0.0177)
              (8,  0.0292)
              (16, 0.0407)
              (32, 0.0598)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.0004)
              (2,  0.0019)
              (4,  0.0033)
              (8,  0.0047)
              (16, 0.0064)
              (32, 0.0084)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.0024)
              (2,  0.0081)
              (4,  0.0162)
              (8,  0.0278)
              (16, 0.0387)
              (32, 0.0552)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  0.0001)
              (8,  0.0002)
              (16, 0.0006)
              (32, 0.0011)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.0000)
              (2,  0.0002)
              (4,  0.0006)
              (8,  0.0015)
              (16, 0.0025)
              (32, 0.0042)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0000)
              (8,  0.0001)
              (16, 0.0002)
              (32, 0.0006)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  -0.0000)
              (2,  0.0001)
              (4,  0.0004)
              (8,  0.0009)
              (16, 0.0016)
              (32, 0.0028)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0001)
              (8,  -0.0000)
              (16, 0.0001)
              (32, 0.0001)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  -0.0000)
              (2,  -0.0000)
              (4,  0.0003)
              (8,  0.0006)
              (16, 0.0011)
              (32, 0.0019)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0000)
              (8,  0.0001)
              (16, 0.0004)
              (32, 0.0010)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0000)
              (8,  0.0002)
              (16, 0.0006)
              (32, 0.0012)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0001)
              (8,  -0.0000)
              (16, 0.0001)
              (32, 0.0004)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0000)
              (8,  0.0002)
              (16, 0.0004)
              (32, 0.0009)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  -0.0000)
              (2,  -0.0001)
              (4,  -0.0001)
              (8,  -0.0001)
              (16, -0.0000)
              (32, 0.0001)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0001)
              (8,  0.0000)
              (16, 0.0002)
              (32, 0.0005)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$}
            
           \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing non-target class drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations. BLIP.}
    \label{fig:deletion_curves_nontarget_drop_blip}
\end{figure}

==> FIGS/corr/blip/overall_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Overall drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]
            
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.0046)
              (2,  0.0078)
              (4,  0.0114)
              (8,  0.0150)
              (16, 0.0194)
              (32, 0.0235)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.0095)
              (2,  0.0176)
              (4,  0.0325)
              (8,  0.0490)
              (16, 0.0629)
              (32, 0.0790)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.0034)
              (2,  0.0059)
              (4,  0.0085)
              (8,  0.0120)
              (16, 0.0142)
              (32, 0.0171)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.0082)
              (2,  0.0155)
              (4,  0.0257)
              (8,  0.0375)
              (16, 0.0492)
              (32, 0.0682)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.0030)
              (2,  0.0053)
              (4,  0.0072)
              (8,  0.0088)
              (16, 0.0109)
              (32, 0.0134)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.0073)
              (2,  0.0147)
              (4,  0.0242)
              (8,  0.0363)
              (16, 0.0473)
              (32, 0.0637)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  0.0004)
              (2,  0.0009)
              (4,  0.0021)
              (8,  0.0039)
              (16, 0.0058)
              (32, 0.0077)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.0009)
              (2,  0.0022)
              (4,  0.0045)
              (8,  0.0075)
              (16, 0.0103)
              (32, 0.0131)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  0.0002)
              (2,  0.0007)
              (4,  0.0018)
              (8,  0.0031)
              (16, 0.0044)
              (32, 0.0058)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  0.0006)
              (2,  0.0016)
              (4,  0.0034)
              (8,  0.0058)
              (16, 0.0085)
              (32, 0.0114)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  0.0001)
              (2,  0.0004)
              (4,  0.0011)
              (8,  0.0020)
              (16, 0.0032)
              (32, 0.0043)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  0.0006)
              (2,  0.0013)
              (4,  0.0028)
              (8,  0.0049)
              (16, 0.0075)
              (32, 0.0102)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  0.0002)
              (2,  0.0005)
              (4,  0.0012)
              (8,  0.0025)
              (16, 0.0050)
              (32, 0.0080)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  0.0003)
              (2,  0.0008)
              (4,  0.0018)
              (8,  0.0036)
              (16, 0.0062)
              (32, 0.0091)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  0.0001)
              (2,  0.0004)
              (4,  0.0009)
              (8,  0.0018)
              (16, 0.0036)
              (32, 0.0058)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  0.0002)
              (2,  0.0006)
              (4,  0.0014)
              (8,  0.0029)
              (16, 0.0051)
              (32, 0.0077)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  0.0001)
              (2,  0.0002)
              (4,  0.0005)
              (8,  0.0011)
              (16, 0.0023)
              (32, 0.0042)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  0.0002)
              (2,  0.0005)
              (4,  0.0011)
              (8,  0.0022)
              (16, 0.0039)
              (32, 0.0064)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$}
  
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing overall drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations. BLIP.}
    \label{fig:deletion_curves_overall_drop_blip}
\end{figure}

==> FIGS/corr/blip/target_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Target drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]
            
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.286)
              (2,  0.334)
              (4,  0.370)
              (8,  0.420)
              (16, 0.485)
              (32, 0.581)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.486)
              (2,  0.680)
              (4,  0.782)
              (8,  0.847)
              (16, 0.878)
              (32, 0.890)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.256)
              (2,  0.376)
              (4,  0.416)
              (8,  0.446)
              (16, 0.489)
              (32, 0.552)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.511)
              (2,  0.710)
              (4,  0.815)
              (8,  0.864)
              (16, 0.889)
              (32, 0.901)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.262)
              (2,  0.344)
              (4,  0.390)
              (8,  0.423)
              (16, 0.456)
              (32, 0.506)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.493)
              (2,  0.671)
              (4,  0.818)
              (8,  0.877)
              (16, 0.902)
              (32, 0.907)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  0.049)
              (2,  0.095)
              (4,  0.207)
              (8,  0.367)
              (16, 0.517)
              (32, 0.662)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.090)
              (2,  0.192)
              (4,  0.384)
              (8,  0.605)
              (16, 0.787)
              (32, 0.895)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  0.028)
              (2,  0.074)
              (4,  0.181)
              (8,  0.301)
              (16, 0.417)
              (32, 0.524)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  0.067)
              (2,  0.153)
              (4,  0.299)
              (8,  0.489)
              (16, 0.699)
              (32, 0.860)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  0.019)
              (2,  0.044)
              (4,  0.119)
              (8,  0.204)
              (16, 0.317)
              (32, 0.418)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  0.061)
              (2,  0.126)
              (4,  0.251)
              (8,  0.429)
              (16, 0.638)
              (32, 0.829)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  0.023)
              (2,  0.053)
              (4,  0.118)
              (8,  0.239)
              (16, 0.459)
              (32, 0.709)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  0.041)
              (2,  0.089)
              (4,  0.181)
              (8,  0.336)
              (16, 0.560)
              (32, 0.789)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  0.020)
              (2,  0.046)
              (4,  0.094)
              (8,  0.188)
              (16, 0.348)
              (32, 0.548)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  0.028)
              (2,  0.069)
              (4,  0.139)
              (8,  0.271)
              (16, 0.465)
              (32, 0.684)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  0.013)
              (2,  0.029)
              (4,  0.060)
              (8,  0.121)
              (16, 0.236)
              (32, 0.410)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  0.033)
              (2,  0.061)
              (4,  0.113)
              (8,  0.218)
              (16, 0.369)
              (32, 0.592)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$} 
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing target class drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations. BLIP.}
    \label{fig:deletion_curves_target_drop_blip}
\end{figure}

==> FIGS/corr/clip/nontarget_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Non-target drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]
            
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.0136)
              (2,  0.0298)
              (4,  0.0700)
              (8,  0.1018)
              (16, 0.1230)
              (32, 0.1355)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.0122)
              (2,  0.0315)
              (4,  0.0769)
              (8,  0.1201)
              (16, 0.1430)
              (32, 0.1682)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.0088)
              (2,  0.0204)
              (4,  0.0440)
              (8,  0.0742)
              (16, 0.0933)
              (32, 0.1065)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.0088)
              (2,  0.0195)
              (4,  0.0422)
              (8,  0.0734)
              (16, 0.0939)
              (32, 0.1099)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.0074)
              (2,  0.0195)
              (4,  0.0381)
              (8,  0.0598)
              (16, 0.0693)
              (32, 0.0763)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.0056)
              (2,  0.0122)
              (4,  0.0299)
              (8,  0.0572)
              (16, 0.0771)
              (32, 0.0931)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  0.0003)
              (2,  0.0010)
              (4,  0.0027)
              (8,  0.0060)
              (16, 0.0120)
              (32, 0.0201)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.0004)
              (2,  0.0011)
              (4,  0.0025)
              (8,  0.0061)
              (16, 0.0122)
              (32, 0.0204)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  0.0001)
              (2,  0.0005)
              (4,  0.0015)
              (8,  0.0036)
              (16, 0.0077)
              (32, 0.0132)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  0.0004)
              (2,  0.0007)
              (4,  0.0020)
              (8,  0.0043)
              (16, 0.0084)
              (32, 0.0126)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  -0.0001)
              (2,  -0.0000)
              (4,  0.0005)
              (8,  0.0015)
              (16, 0.0038)
              (32, 0.0072)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  0.0000)
              (2,  0.0004)
              (4,  0.0010)
              (8,  0.0025)
              (16, 0.0046)
              (32, 0.0069)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  0.0001)
              (2,  0.0003)
              (4,  0.0012)
              (8,  0.0026)
              (16, 0.0053)
              (32, 0.0098)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  -0.0000)
              (2,  0.0001)
              (4,  0.0007)
              (8,  0.0022)
              (16, 0.0050)
              (32, 0.0092)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  -0.0001)
              (2,  -0.0000)
              (4,  0.0002)
              (8,  0.0008)
              (16, 0.0018)
              (32, 0.0039)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  -0.0001)
              (2,  -0.0000)
              (4,  0.0003)
              (8,  0.0008)
              (16, 0.0023)
              (32, 0.0047)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  -0.0001)
              (2,  -0.0002)
              (4,  -0.0001)
              (8,  0.0001)
              (16, 0.0007)
              (32, 0.0018)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  -0.0001)
              (2,  -0.0001)
              (4,  -0.0000)
              (8,  0.0004)
              (16, 0.0011)
              (32, 0.0022)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$}
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing non-target class drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations.  CLIP.}
    \label{fig:deletion_curves_nontarget_drop_clip}
\end{figure}

==> FIGS/corr/clip/overall_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Overall drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]
            
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.0169)
              (2,  0.0336)
              (4,  0.0740)
              (8,  0.1060)
              (16, 0.1276)
              (32, 0.1408)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.0167)
              (2,  0.0370)
              (4,  0.0826)
              (8,  0.1256)
              (16, 0.1483)
              (32, 0.1734)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.0117)
              (2,  0.0238)
              (4,  0.0475)
              (8,  0.0777)
              (16, 0.0970)
              (32, 0.1103)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.0133)
              (2,  0.0250)
              (4,  0.0481)
              (8,  0.0794)
              (16, 0.0998)
              (32, 0.1157)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.0100)
              (2,  0.0223)
              (4,  0.0410)
              (8,  0.0626)
              (16, 0.0723)
              (32, 0.0796)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.0098)
              (2,  0.0178)
              (4,  0.0362)
              (8,  0.0637)
              (16, 0.0835)
              (32, 0.0994)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  0.0023)
              (2,  0.0047)
              (4,  0.0085)
              (8,  0.0132)
              (16, 0.0199)
              (32, 0.0284)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.0025)
              (2,  0.0049)
              (4,  0.0085)
              (8,  0.0137)
              (16, 0.0204)
              (32, 0.0286)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  0.0017)
              (2,  0.0033)
              (4,  0.0060)
              (8,  0.0096)
              (16, 0.0145)
              (32, 0.0208)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  0.0022)
              (2,  0.0040)
              (4,  0.0072)
              (8,  0.0113)
              (16, 0.0162)
              (32, 0.0208)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  0.0009)
              (2,  0.0020)
              (4,  0.0042)
              (8,  0.0066)
              (16, 0.0098)
              (32, 0.0137)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  0.0014)
              (2,  0.0030)
              (4,  0.0055)
              (8,  0.0089)
              (16, 0.0119)
              (32, 0.0149)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  0.0011)
              (2,  0.0023)
              (4,  0.0049)
              (8,  0.0087)
              (16, 0.0130)
              (32, 0.0183)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  0.0010)
              (2,  0.0021)
              (4,  0.0045)
              (8,  0.0082)
              (16, 0.0128)
              (32, 0.0177)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  0.0005)
              (2,  0.0013)
              (4,  0.0026)
              (8,  0.0052)
              (16, 0.0083)
              (32, 0.0118)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  0.0006)
              (2,  0.0013)
              (4,  0.0028)
              (8,  0.0054)
              (16, 0.0088)
              (32, 0.0126)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  0.0003)
              (2,  0.0007)
              (4,  0.0016)
              (8,  0.0032)
              (16, 0.0055)
              (32, 0.0082)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  0.0004)
              (2,  0.0009)
              (4,  0.0019)
              (8,  0.0038)
              (16, 0.0064)
              (32, 0.0091)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$} 
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing overall drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations.  CLIP.}
    \label{fig:deletion_curves_overall_drop_clip}
\end{figure}

==> FIGS/corr/clip/target_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Target drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]
            
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.342)
              (2,  0.415)
              (4,  0.474)
              (8,  0.529)
              (16, 0.592)
              (32, 0.666)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.470)
              (2,  0.575)
              (4,  0.642)
              (8,  0.668)
              (16, 0.678)
              (32, 0.682)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.298)
              (2,  0.353)
              (4,  0.395)
              (8,  0.431)
              (16, 0.463)
              (32, 0.493)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.459)
              (2,  0.572)
              (4,  0.639)
              (8,  0.671)
              (16, 0.683)
              (32, 0.688)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.261)
              (2,  0.304)
              (4,  0.326)
              (8,  0.348)
              (16, 0.374)
              (32, 0.404)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.423)
              (2,  0.567)
              (4,  0.658)
              (8,  0.700)
              (16, 0.713)
              (32, 0.718)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  0.202)
              (2,  0.371)
              (4,  0.587)
              (8,  0.726)
              (16, 0.806)
              (32, 0.853)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.207)
              (2,  0.383)
              (4,  0.603)
              (8,  0.765)
              (16, 0.829)
              (32, 0.849)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  0.154)
              (2,  0.276)
              (4,  0.456)
              (8,  0.597)
              (16, 0.696)
              (32, 0.769)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  0.184)
              (2,  0.332)
              (4,  0.526)
              (8,  0.706)
              (16, 0.792)
              (32, 0.830)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  0.106)
              (2,  0.206)
              (4,  0.370)
              (8,  0.509)
              (16, 0.595)
              (32, 0.663)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  0.138)
              (2,  0.265)
              (4,  0.456)
              (8,  0.639)
              (16, 0.741)
              (32, 0.799)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  0.097)
              (2,  0.193)
              (4,  0.371)
              (8,  0.605)
              (16, 0.770)
              (32, 0.857)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  0.101)
              (2,  0.199)
              (4,  0.379)
              (8,  0.611)
              (16, 0.781)
              (32, 0.858)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  0.064)
              (2,  0.130)
              (4,  0.241)
              (8,  0.445)
              (16, 0.643)
              (32, 0.795)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  0.068)
              (2,  0.132)
              (4,  0.249)
              (8,  0.457)
              (16, 0.650)
              (32, 0.799)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  0.041)
              (2,  0.084)
              (4,  0.171)
              (8,  0.301)
              (16, 0.474)
              (32, 0.639)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  0.056)
              (2,  0.102)
              (4,  0.191)
              (8,  0.340)
              (16, 0.531)
              (32, 0.695)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$}
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing target class drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations. CLIP.}
    \label{fig:deletion_curves_target_drop_clip}
\end{figure}

==> FIGS/corr/combined_target.tex <==
\begin{figure*}[t]
    \centering
    %% ===================== ROW 1: TopKSAE (dashed) =====================
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={(a) Target drop -- TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 legend to name=legendTopK,
                 legend style={legend columns=3, font=\scriptsize, column sep=0.3cm},
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,0.06451)(2,0.14111)(4,0.29186)(8,0.60043)(16,0.82120)(32,0.88980)
                };
                \addlegendentry{TopK\_l1536\_k10}
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,0.04897)(2,0.10674)(4,0.22006)(8,0.50889)(16,0.75246)(32,0.87160)
                };
                \addlegendentry{TopK\_l3072\_k10}
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,0.04491)(2,0.09769)(4,0.21774)(8,0.45734)(16,0.70703)(32,0.84709)
                };
                \addlegendentry{TopK\_l6144\_k10}
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,0.02997)(2,0.05989)(4,0.14037)(8,0.29374)(16,0.57934)(32,0.84246)
                };
                \addlegendentry{TopK\_l1536\_k32}
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,0.02000)(2,0.04757)(4,0.09557)(8,0.20814)(16,0.49254)(32,0.76623)
                };
                \addlegendentry{TopK\_l3072\_k32}
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,0.01860)(2,0.03660)(4,0.07686)(8,0.18606)(16,0.43400)(32,0.71203)
                };
                \addlegendentry{TopK\_l6144\_k32}
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,0.02294)(2,0.04571)(4,0.09377)(8,0.19506)(16,0.39689)(32,0.68403)
                };
                \addlegendentry{TopK\_l1536\_k64}
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,0.01589)(2,0.03234)(4,0.07137)(8,0.15106)(16,0.31566)(32,0.62643)
                };
                \addlegendentry{TopK\_l3072\_k64}
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,0.01174)(2,0.02269)(4,0.05140)(8,0.11200)(16,0.25637)(32,0.51940)
                };
                \addlegendentry{TopK\_l6144\_k64}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={(b) Overall drop -- TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,0.000511)(2,0.001285)(4,0.002968)(8,0.006614)(16,0.010236)(32,0.012950)
                };
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,0.000413)(2,0.000991)(4,0.002191)(8,0.005532)(16,0.008714)(32,0.011267)
                };
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,0.000380)(2,0.000889)(4,0.002084)(8,0.004823)(16,0.008064)(32,0.010606)
                };
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,0.000233)(2,0.000475)(4,0.001249)(8,0.003000)(16,0.006490)(32,0.010327)
                };
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,0.000125)(2,0.000341)(4,0.000772)(8,0.001974)(16,0.005078)(32,0.008554)
                };
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,0.000104)(2,0.000253)(4,0.000633)(8,0.001724)(16,0.004385)(32,0.007625)
                };
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,0.000105)(2,0.000292)(4,0.000717)(8,0.001818)(16,0.004163)(32,0.007993)
                };
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,0.000088)(2,0.000199)(4,0.000546)(8,0.001353)(16,0.003210)(32,0.006857)
                };
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,0.000041)(2,0.000110)(4,0.000335)(8,0.000898)(16,0.002358)(32,0.005186)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={(c) Non-target drop -- TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,-0.000135)(2,-0.000127)(4,0.000050)(8,0.000616)(16,0.002045)(32,0.004093)
                };
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,-0.000077)(2,-0.000077)(4,-0.000010)(8,0.000448)(16,0.001202)(32,0.002576)
                };
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,-0.000070)(2,-0.000089)(4,-0.000094)(8,0.000253)(16,0.001003)(32,0.002157)
                };
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,-0.000067)(2,-0.000125)(4,-0.000157)(8,0.000063)(16,0.000704)(32,0.001921)
                };
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,-0.000076)(2,-0.000137)(4,-0.000186)(8,-0.000109)(16,0.000154)(32,0.000900)
                };
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,-0.000083)(2,-0.000114)(4,-0.000137)(8,-0.000138)(16,0.000046)(32,0.000510)
                };
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,-0.000126)(2,-0.000167)(4,-0.000223)(8,-0.000134)(16,0.000196)(32,0.001164)
                };
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,-0.000072)(2,-0.000126)(4,-0.000170)(8,-0.000159)(16,0.000054)(32,0.000599)
                };
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,-0.000077)(2,-0.000118)(4,-0.000181)(8,-0.000224)(16,-0.000208)(32,-0.000008)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}

    \vspace{0.4em}

    %% ===================== ROW 2: BatchTopKSAE (solid) =====================
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={(d) Target drop -- BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 legend to name=legendBatch,
                 legend style={legend columns=3, font=\scriptsize, column sep=0.3cm},
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,0.04969)(2,0.10334)(4,0.24420)(8,0.58203)(16,0.79509)(32,0.85169)
                };
                \addlegendentry{BatchTopK\_l1536\_k10}
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,0.02974)(2,0.07529)(4,0.17831)(8,0.44440)(16,0.70034)(32,0.78763)
                };
                \addlegendentry{BatchTopK\_l3072\_k10}
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,0.03249)(2,0.06569)(4,0.14463)(8,0.40517)(16,0.65169)(32,0.76911)
                };
                \addlegendentry{BatchTopK\_l6144\_k10}
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,0.03109)(2,0.07129)(4,0.15334)(8,0.28643)(16,0.53686)(32,0.81640)
                };
                \addlegendentry{BatchTopK\_l1536\_k32}
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,0.02234)(2,0.04154)(4,0.09191)(8,0.20177)(16,0.44834)(32,0.74977)
                };
                \addlegendentry{BatchTopK\_l3072\_k32}
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,0.01534)(2,0.03163)(4,0.06823)(8,0.15140)(16,0.36940)(32,0.65477)
                };
                \addlegendentry{BatchTopK\_l6144\_k32}
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,0.02083)(2,0.04500)(4,0.09837)(8,0.20271)(16,0.40337)(32,0.70714)
                };
                \addlegendentry{BatchTopK\_l1536\_k64}
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,0.01560)(2,0.03146)(4,0.06583)(8,0.12717)(16,0.30046)(32,0.60920)
                };
                \addlegendentry{BatchTopK\_l3072\_k64}
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,0.01186)(2,0.02414)(4,0.04937)(8,0.10357)(16,0.25349)(32,0.52974)
                };
                \addlegendentry{BatchTopK\_l6144\_k64}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={(e) Overall drop -- BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,0.000403)(2,0.000901)(4,0.002375)(8,0.006201)(16,0.009466)(32,0.012347)
                };
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,0.000202)(2,0.000591)(4,0.001589)(8,0.004415)(16,0.007571)(32,0.009646)
                };
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,0.000211)(2,0.000475)(4,0.001229)(8,0.003874)(16,0.006705)(32,0.008560)
                };
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,0.000192)(2,0.000525)(4,0.001351)(8,0.002871)(16,0.005996)(32,0.009888)
                };
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,0.000121)(2,0.000279)(4,0.000732)(8,0.001855)(16,0.004565)(32,0.008142)
                };
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,0.000086)(2,0.000205)(4,0.000524)(8,0.001334)(16,0.003604)(32,0.006881)
                };
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,0.000143)(2,0.000341)(4,0.000886)(8,0.002027)(16,0.004457)(32,0.008562)
                };
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,0.000069)(2,0.000179)(4,0.000459)(8,0.001040)(16,0.002980)(32,0.006405)
                };
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,0.000040)(2,0.000117)(4,0.000312)(8,0.000831)(16,0.002394)(32,0.005429)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={(f) Non-target drop -- BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,-0.000095)(2,-0.000134)(4,-0.000068)(8,0.000384)(16,0.001530)(32,0.003868)
                };
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,-0.000096)(2,-0.000164)(4,-0.000196)(8,-0.000029)(16,0.000574)(32,0.001788)
                };
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,-0.000115)(2,-0.000184)(4,-0.000220)(8,-0.000180)(16,0.000190)(32,0.000878)
                };
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,-0.000120)(2,-0.000190)(4,-0.000184)(8,0.000007)(16,0.000633)(32,0.001742)
                };
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,-0.000103)(2,-0.000138)(4,-0.000189)(8,-0.000165)(16,0.000083)(32,0.000651)
                };
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,-0.000068)(2,-0.000113)(4,-0.000160)(8,-0.000182)(16,-0.000091)(32,0.000337)
                };
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,-0.000066)(2,-0.000111)(4,-0.000099)(8,0.000000)(16,0.000427)(32,0.001505)
                };
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,-0.000088)(2,-0.000137)(4,-0.000201)(8,-0.000234)(16,-0.000025)(32,0.000316)
                };
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,-0.000079)(2,-0.000126)(4,-0.000184)(8,-0.000207)(16,-0.000143)(32,0.000133)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}

    \vspace{0.3em}
    \ref{legendTopK}\par\vspace{0.2em}
    \ref{legendBatch}
    
    \caption{Deletion curves showing target drop (a,d), overall drop (b,e), and non-target drop (c,f) as a function of number of deleted features (N). Top row: TopKSAE, bottom row: BatchTopKSAE. DINO.}
    \label{fig:deletion_curves_combined_dino}
\end{figure*}

==> FIGS/corr/dino/nontarget_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Non-target drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]
            
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  -0.000095)
              (2,  -0.000134)
              (4,  -0.000068)
              (8,  0.000384)
              (16, 0.001530)
              (32, 0.003868)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  -0.000135)
              (2,  -0.000127)
              (4,  0.000050)
              (8,  0.000616)
              (16, 0.002045)
              (32, 0.004093)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  -0.000096)
              (2,  -0.000164)
              (4,  -0.000196)
              (8,  -0.000029)
              (16, 0.000574)
              (32, 0.001788)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  -0.000077)
              (2,  -0.000077)
              (4,  -0.000010)
              (8,  0.000448)
              (16, 0.001202)
              (32, 0.002576)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  -0.000115)
              (2,  -0.000184)
              (4,  -0.000220)
              (8,  -0.000180)
              (16, 0.000190)
              (32, 0.000878)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  -0.000070)
              (2,  -0.000089)
              (4,  -0.000094)
              (8,  0.000253)
              (16, 0.001003)
              (32, 0.002157)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  -0.000120)
              (2,  -0.000190)
              (4,  -0.000184)
              (8,  0.000007)
              (16, 0.000633)
              (32, 0.001742)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  -0.000067)
              (2,  -0.000125)
              (4,  -0.000157)
              (8,  0.000063)
              (16, 0.000704)
              (32, 0.001921)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  -0.000103)
              (2,  -0.000138)
              (4,  -0.000189)
              (8,  -0.000165)
              (16, 0.000083)
              (32, 0.000651)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  -0.000076)
              (2,  -0.000137)
              (4,  -0.000186)
              (8,  -0.000109)
              (16, 0.000154)
              (32, 0.000900)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  -0.000068)
              (2,  -0.000113)
              (4,  -0.000160)
              (8,  -0.000182)
              (16, -0.000091)
              (32, 0.000337)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  -0.000083)
              (2,  -0.000114)
              (4,  -0.000137)
              (8,  -0.000138)
              (16, 0.000046)
              (32, 0.000510)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  -0.000066)
              (2,  -0.000111)
              (4,  -0.000099)
              (8,  0.000000)
              (16, 0.000427)
              (32, 0.001505)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  -0.000126)
              (2,  -0.000167)
              (4,  -0.000223)
              (8,  -0.000134)
              (16, 0.000196)
              (32, 0.001164)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  -0.000088)
              (2,  -0.000137)
              (4,  -0.000201)
              (8,  -0.000234)
              (16, -0.000025)
              (32, 0.000316)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  -0.000072)
              (2,  -0.000126)
              (4,  -0.000170)
              (8,  -0.000159)
              (16, 0.000054)
              (32, 0.000599)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  -0.000079)
              (2,  -0.000126)
              (4,  -0.000184)
              (8,  -0.000207)
              (16, -0.000143)
              (32, 0.000133)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  -0.000077)
              (2,  -0.000118)
              (4,  -0.000181)
              (8,  -0.000224)
              (16, -0.000208)
              (32, -0.000008)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$} 
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing non-target class drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations. DINO.}
    \label{fig:deletion_curves_nontarget_drop_dino}
\end{figure}

==> FIGS/corr/dino/overall_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
                     width=\linewidth,
                     xlabel=Number of deleted features (N), 
                     ylabel=Overall drop,
                     grid=both,
                     grid style={line width=.1pt, dashed, draw=gray!10},
                     major grid style={line width=.2pt,draw=gray!50},
                     xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
                     ]

            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.000403)
              (2,  0.000901)
              (4,  0.002375)
              (8,  0.006201)
              (16, 0.009466)
              (32, 0.012347)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.000511)
              (2,  0.001285)
              (4,  0.002968)
              (8,  0.006614)
              (16, 0.010236)
              (32, 0.012950)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.000202)
              (2,  0.000591)
              (4,  0.001589)
              (8,  0.004415)
              (16, 0.007571)
              (32, 0.009646)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.000413)
              (2,  0.000991)
              (4,  0.002191)
              (8,  0.005532)
              (16, 0.008714)
              (32, 0.011267)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.000211)
              (2,  0.000475)
              (4,  0.001229)
              (8,  0.003874)
              (16, 0.006705)
              (32, 0.008560)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.000380)
              (2,  0.000889)
              (4,  0.002084)
              (8,  0.004823)
              (16, 0.008064)
              (32, 0.010606)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  0.000192)
              (2,  0.000525)
              (4,  0.001351)
              (8,  0.002871)
              (16, 0.005996)
              (32, 0.009888)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.000233)
              (2,  0.000475)
              (4,  0.001249)
              (8,  0.003000)
              (16, 0.006490)
              (32, 0.010327)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  0.000121)
              (2,  0.000279)
              (4,  0.000732)
              (8,  0.001855)
              (16, 0.004565)
              (32, 0.008142)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  0.000125)
              (2,  0.000341)
              (4,  0.000772)
              (8,  0.001974)
              (16, 0.005078)
              (32, 0.008554)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  0.000086)
              (2,  0.000205)
              (4,  0.000524)
              (8,  0.001334)
              (16, 0.003604)
              (32, 0.006881)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  0.000104)
              (2,  0.000253)
              (4,  0.000633)
              (8,  0.001724)
              (16, 0.004385)
              (32, 0.007625)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  0.000143)
              (2,  0.000341)
              (4,  0.000886)
              (8,  0.002027)
              (16, 0.004457)
              (32, 0.008562)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  0.000105)
              (2,  0.000292)
              (4,  0.000717)
              (8,  0.001818)
              (16, 0.004163)
              (32, 0.007993)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  0.000069)
              (2,  0.000179)
              (4,  0.000459)
              (8,  0.001040)
              (16, 0.002980)
              (32, 0.006405)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  0.000088)
              (2,  0.000199)
              (4,  0.000546)
              (8,  0.001353)
              (16, 0.003210)
              (32, 0.006857)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  0.000040)
              (2,  0.000117)
              (4,  0.000312)
              (8,  0.000831)
              (16, 0.002394)
              (32, 0.005429)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  0.000041)
              (2,  0.000110)
              (4,  0.000335)
              (8,  0.000898)
              (16, 0.002358)
              (32, 0.005186)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$}
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing overall drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations. DINO.}
    \label{fig:deletion_curves_overall_drop_dino}
\end{figure}

==> FIGS/corr/dino/target_drop_plot.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale = 0.95]
        \begin{axis}[legend style={at={(0.5,-0.2)}, anchor=north, legend columns=2, font=\footnotesize, column sep=1cm},
             width=\linewidth,
             xlabel=Number of deleted features (N), 
             ylabel=Target drop,  % ZMIEŃ NA: Overall drop / Non-target drop
             grid=both,
             grid style={line width=.1pt, dashed, draw=gray!10},
             major grid style={line width=.2pt,draw=gray!50},
             xmode=log,
             log basis x=2,
             xtick={1,2,4,8,16,32},
             xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$}
             ]     
            % BatchTopKSAE models (solid lines)
            \addplot[color=red, mark=square*, solid] coordinates {    % BatchTopKSAE_l1536_k10
              (1,  0.04969)
              (2,  0.10334)
              (4,  0.24420)
              (8,  0.58203)
              (16, 0.79509)
              (32, 0.85169)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k10$}

            \addplot[color=red, mark=square*, dashed] coordinates {    % TopKSAE_l1536_k10
              (1,  0.06451)
              (2,  0.14111)
              (4,  0.29186)
              (8,  0.60043)
              (16, 0.82120)
              (32, 0.88980)
            };
            \addlegendentry{$TopKSAE\_l1536\_k10$}
            
            \addplot[color=blue, mark=square*, solid] coordinates {   % BatchTopKSAE_l3072_k10
              (1,  0.02974)
              (2,  0.07529)
              (4,  0.17831)
              (8,  0.44440)
              (16, 0.70034)
              (32, 0.78763)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k10$}

            \addplot[color=blue, mark=square*, dashed] coordinates {   % TopKSAE_l3072_k10
              (1,  0.04897)
              (2,  0.10674)
              (4,  0.22006)
              (8,  0.50889)
              (16, 0.75246)
              (32, 0.87160)
            };
            \addlegendentry{$TopKSAE\_l3072\_k10$}
            
            \addplot[color=green!50!black, mark=square*, solid] coordinates {  % BatchTopKSAE_l6144_k10
              (1,  0.03249)
              (2,  0.06569)
              (4,  0.14463)
              (8,  0.40517)
              (16, 0.65169)
              (32, 0.76911)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k10$}

            \addplot[color=green!50!black, mark=square*, dashed] coordinates { % TopKSAE_l6144_k10
              (1,  0.04491)
              (2,  0.09769)
              (4,  0.21774)
              (8,  0.45734)
              (16, 0.70703)
              (32, 0.84709)
            };
            \addlegendentry{$TopKSAE\_l6144\_k10$}
            
            \addplot[color=red, mark=triangle*, solid] coordinates {   % BatchTopKSAE_l1536_k32
              (1,  0.03109)
              (2,  0.07129)
              (4,  0.15334)
              (8,  0.28643)
              (16, 0.53686)
              (32, 0.81640)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k32$}

            \addplot[color=red, mark=triangle*, dashed] coordinates {   % TopKSAE_l1536_k32
              (1,  0.02997)
              (2,  0.05989)
              (4,  0.14037)
              (8,  0.29374)
              (16, 0.57934)
              (32, 0.84246)
            };
            \addlegendentry{$TopKSAE\_l1536\_k32$}
            
            \addplot[color=blue, mark=triangle*, solid] coordinates {  % BatchTopKSAE_l3072_k32
              (1,  0.02234)
              (2,  0.04154)
              (4,  0.09191)
              (8,  0.20177)
              (16, 0.44834)
              (32, 0.74977)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k32$}

            \addplot[color=blue, mark=triangle*, dashed] coordinates {  % TopKSAE_l3072_k32
              (1,  0.02000)
              (2,  0.04757)
              (4,  0.09557)
              (8,  0.20814)
              (16, 0.49254)
              (32, 0.76623)
            };
            \addlegendentry{$TopKSAE\_l3072\_k32$}
            
            \addplot[color=green!50!black, mark=triangle*, solid] coordinates { % BatchTopKSAE_l6144_k32
              (1,  0.01534)
              (2,  0.03163)
              (4,  0.06823)
              (8,  0.15140)
              (16, 0.36940)
              (32, 0.65477)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k32$}

            \addplot[color=green!50!black, mark=triangle*, dashed] coordinates { % TopKSAE_l6144_k32
              (1,  0.01860)
              (2,  0.03660)
              (4,  0.07686)
              (8,  0.18606)
              (16, 0.43400)
              (32, 0.71203)
            };
            \addlegendentry{$TopKSAE\_l6144\_k32$}
            
            \addplot[color=red, mark=diamond*, solid] coordinates {    % BatchTopKSAE_l1536_k64
              (1,  0.02083)
              (2,  0.04500)
              (4,  0.09837)
              (8,  0.20271)
              (16, 0.40337)
              (32, 0.70714)
            };
            \addlegendentry{$BatchTopKSAE\_l1536\_k64$}

            \addplot[color=red, mark=diamond*, dashed] coordinates {    % TopKSAE_l1536_k64
              (1,  0.02294)
              (2,  0.04571)
              (4,  0.09377)
              (8,  0.19506)
              (16, 0.39689)
              (32, 0.68403)
            };
            \addlegendentry{$TopKSAE\_l1536\_k64$}
            
            \addplot[color=blue, mark=diamond*, solid] coordinates {   % BatchTopKSAE_l3072_k64
              (1,  0.01560)
              (2,  0.03146)
              (4,  0.06583)
              (8,  0.12717)
              (16, 0.30046)
              (32, 0.60920)
            };
            \addlegendentry{$BatchTopKSAE\_l3072\_k64$}

            \addplot[color=blue, mark=diamond*, dashed] coordinates {   % TopKSAE_l3072_k64
              (1,  0.01589)
              (2,  0.03234)
              (4,  0.07137)
              (8,  0.15106)
              (16, 0.31566)
              (32, 0.62643)
            };
            \addlegendentry{$TopKSAE\_l3072\_k64$}
            
            \addplot[color=green!50!black, mark=diamond*, solid] coordinates { % BatchTopKSAE_l6144_k64
              (1,  0.01186)
              (2,  0.02414)
              (4,  0.04937)
              (8,  0.10357)
              (16, 0.25349)
              (32, 0.52974)
            };
            \addlegendentry{$BatchTopKSAE\_l6144\_k64$}

            \addplot[color=green!50!black, mark=diamond*, dashed] coordinates { % TopKSAE_l6144_k64
              (1,  0.01174)
              (2,  0.02269)
              (4,  0.05140)
              (8,  0.11200)
              (16, 0.25637)
              (32, 0.51940)
            };
            \addlegendentry{$TopKSAE\_l6144\_k64$} 
        \end{axis}
    \end{tikzpicture}
    \caption{Deletion curves showing target class drop as a function of number of deleted features (N) for BatchTopKSAE and TopKSAE models with various configurations. DINO.}
    \label{fig:deletion_curves_target_drop_dino}
\end{figure}

==> FIGS/corr/nontarget_drop_combined_plot.tex <==
\begin{figure*}[t]
    \centering
    %% ===================== ROW 1: TopKSAE =====================
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={DINO: TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 legend to name=legendTopK,
                 legend style={legend columns=3, font=\scriptsize, column sep=0.3cm},
                 scaled y ticks=false
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,-0.000135)(2,-0.000127)(4,5e-05)(8,0.000616)(16,0.002045)(32,0.004093)
                };
                \addlegendentry{TopK\_l1536\_k10}
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,-7.7e-05)(2,-7.7e-05)(4,-1e-05)(8,0.000448)(16,0.001202)(32,0.002576)
                };
                \addlegendentry{TopK\_l3072\_k10}
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,-7e-05)(2,-8.9e-05)(4,-9.4e-05)(8,0.000253)(16,0.001003)(32,0.002157)
                };
                \addlegendentry{TopK\_l6144\_k10}
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,-6.7e-05)(2,-0.000125)(4,-0.000157)(8,6.3e-05)(16,0.000704)(32,0.001921)
                };
                \addlegendentry{TopK\_l1536\_k32}
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,-7.6e-05)(2,-0.000137)(4,-0.000186)(8,-0.000109)(16,0.000154)(32,0.0009)
                };
                \addlegendentry{TopK\_l3072\_k32}
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,-8.3e-05)(2,-0.000114)(4,-0.000137)(8,-0.000138)(16,4.6e-05)(32,0.00051)
                };
                \addlegendentry{TopK\_l6144\_k32}
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,-0.000126)(2,-0.000167)(4,-0.000223)(8,-0.000134)(16,0.000196)(32,0.001164)
                };
                \addlegendentry{TopK\_l1536\_k64}
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,-7.2e-05)(2,-0.000126)(4,-0.00017)(8,-0.000159)(16,5.4e-05)(32,0.000599)
                };
                \addlegendentry{TopK\_l3072\_k64}
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,-7.7e-05)(2,-0.000118)(4,-0.000181)(8,-0.000224)(16,-0.000208)(32,-8e-06)
                };
                \addlegendentry{TopK\_l6144\_k64}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={CLIP: TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 scaled y ticks=false
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,0.0122)(2,0.0315)(4,0.0769)(8,0.1201)(16,0.143)(32,0.1682)
                };
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,0.0088)(2,0.0195)(4,0.0422)(8,0.0734)(16,0.0939)(32,0.1099)
                };
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,0.0056)(2,0.0122)(4,0.0299)(8,0.0572)(16,0.0771)(32,0.0931)
                };
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,0.0004)(2,0.0011)(4,0.0025)(8,0.0061)(16,0.0122)(32,0.0204)
                };
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,0.0004)(2,0.0007)(4,0.002)(8,0.0043)(16,0.0084)(32,0.0126)
                };
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,0.0)(2,0.0004)(4,0.001)(8,0.0025)(16,0.0046)(32,0.0069)
                };
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,-0.0)(2,0.0001)(4,0.0007)(8,0.0022)(16,0.005)(32,0.0092)
                };
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,-0.0001)(2,-0.0)(4,0.0003)(8,0.0008)(16,0.0023)(32,0.0047)
                };
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0)(8,0.0004)(16,0.0011)(32,0.0022)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={BLIP: TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 scaled y ticks=false
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,0.0047)(2,0.0109)(4,0.025)(8,0.041)(16,0.0547)(32,0.0708)
                };
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,0.0032)(2,0.0085)(4,0.0177)(8,0.0292)(16,0.0407)(32,0.0598)
                };
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,0.0024)(2,0.0081)(4,0.0162)(8,0.0278)(16,0.0387)(32,0.0552)
                };
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,0.0)(2,0.0002)(4,0.0006)(8,0.0015)(16,0.0025)(32,0.0042)
                };
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,-0.0)(2,0.0001)(4,0.0004)(8,0.0009)(16,0.0016)(32,0.0028)
                };
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,-0.0)(2,-0.0)(4,0.0003)(8,0.0006)(16,0.0011)(32,0.0019)
                };
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0)(8,0.0002)(16,0.0006)(32,0.0012)
                };
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0)(8,0.0002)(16,0.0004)(32,0.0009)
                };
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0001)(8,0.0)(16,0.0002)(32,0.0005)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}

    \vspace{0.4em}

    %% ===================== ROW 2: BatchTopKSAE =====================
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={DINO: BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 legend to name=legendBatch,
                 legend style={legend columns=3, font=\scriptsize, column sep=0.3cm},
                 scaled y ticks=false
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,-9.5e-05)(2,-0.000134)(4,-6.8e-05)(8,0.000384)(16,0.00153)(32,0.003868)
                };
                \addlegendentry{BatchTopK\_l1536\_k10}
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,-9.6e-05)(2,-0.000164)(4,-0.000196)(8,-2.9e-05)(16,0.000574)(32,0.001788)
                };
                \addlegendentry{BatchTopK\_l3072\_k10}
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,-0.000115)(2,-0.000184)(4,-0.00022)(8,-0.00018)(16,0.00019)(32,0.000878)
                };
                \addlegendentry{BatchTopK\_l6144\_k10}
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,-0.00012)(2,-0.00019)(4,-0.000184)(8,7e-06)(16,0.000633)(32,0.001742)
                };
                \addlegendentry{BatchTopK\_l1536\_k32}
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,-0.000103)(2,-0.000138)(4,-0.000189)(8,-0.000165)(16,8.3e-05)(32,0.000651)
                };
                \addlegendentry{BatchTopK\_l3072\_k32}
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,-6.8e-05)(2,-0.000113)(4,-0.00016)(8,-0.000182)(16,-9.1e-05)(32,0.000337)
                };
                \addlegendentry{BatchTopK\_l6144\_k32}
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,-6.6e-05)(2,-0.000111)(4,-9.9e-05)(8,0.0)(16,0.000427)(32,0.001505)
                };
                \addlegendentry{BatchTopK\_l1536\_k64}
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,-8.8e-05)(2,-0.000137)(4,-0.000201)(8,-0.000234)(16,-2.5e-05)(32,0.000316)
                };
                \addlegendentry{BatchTopK\_l3072\_k64}
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,-7.9e-05)(2,-0.000126)(4,-0.000184)(8,-0.000207)(16,-0.000143)(32,0.000133)
                };
                \addlegendentry{BatchTopK\_l6144\_k64}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={CLIP: BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 scaled y ticks=false
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,0.0136)(2,0.0298)(4,0.07)(8,0.1018)(16,0.123)(32,0.1355)
                };
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,0.0088)(2,0.0204)(4,0.044)(8,0.0742)(16,0.0933)(32,0.1065)
                };
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,0.0074)(2,0.0195)(4,0.0381)(8,0.0598)(16,0.0693)(32,0.0763)
                };
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,0.0003)(2,0.001)(4,0.0027)(8,0.006)(16,0.012)(32,0.0201)
                };
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,0.0001)(2,0.0005)(4,0.0015)(8,0.0036)(16,0.0077)(32,0.0132)
                };
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,-0.0001)(2,-0.0)(4,0.0005)(8,0.0015)(16,0.0038)(32,0.0072)
                };
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,0.0001)(2,0.0003)(4,0.0012)(8,0.0026)(16,0.0053)(32,0.0098)
                };
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,-0.0001)(2,-0.0)(4,0.0002)(8,0.0008)(16,0.0018)(32,0.0039)
                };
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,-0.0001)(2,-0.0002)(4,-0.0001)(8,0.0001)(16,0.0007)(32,0.0018)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Non-target drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={BLIP: BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 scaled y ticks=false
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,0.0017)(2,0.0045)(4,0.0077)(8,0.0109)(16,0.0147)(32,0.0179)
                };
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,0.0009)(2,0.0022)(4,0.0044)(8,0.0076)(16,0.0094)(32,0.0117)
                };
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,0.0004)(2,0.0019)(4,0.0033)(8,0.0047)(16,0.0064)(32,0.0084)
                };
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,0.0001)(8,0.0002)(16,0.0006)(32,0.0011)
                };
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0)(8,0.0001)(16,0.0002)(32,0.0006)
                };
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0001)(8,-0.0)(16,0.0001)(32,0.0001)
                };
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0)(8,0.0001)(16,0.0004)(32,0.001)
                };
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,-0.0001)(2,-0.0001)(4,-0.0001)(8,-0.0)(16,0.0001)(32,0.0004)
                };
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,-0.0)(2,-0.0001)(4,-0.0001)(8,-0.0001)(16,-0.0)(32,0.0001)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}

    \vspace{0.3em}
    \ref{legendTopK}\par\vspace{0.2em}
    \ref{legendBatch}

    \caption{Deletion curves showing non-target drop as a function of number of deleted features (N). Top row: TopKSAE, bottom row: BatchTopKSAE. Columns: DINO, CLIP, BLIP.}
    \label{fig:deletion_curves_nontarget_per_metric}
\end{figure*}

==> FIGS/corr/overall_drop_combined_plot.tex <==
\begin{figure*}[t]
    \centering
    %% ===================== ROW 1: TopKSAE =====================
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={DINO: TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 legend to name=legendTopK,
                 legend style={legend columns=3, font=\scriptsize, column sep=0.3cm},
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,0.000511)(2,0.001285)(4,0.002968)(8,0.006614)(16,0.010236)(32,0.01295)
                };
                \addlegendentry{TopK\_l1536\_k10}
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,0.000413)(2,0.000991)(4,0.002191)(8,0.005532)(16,0.008714)(32,0.011267)
                };
                \addlegendentry{TopK\_l3072\_k10}
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,0.00038)(2,0.000889)(4,0.002084)(8,0.004823)(16,0.008064)(32,0.010606)
                };
                \addlegendentry{TopK\_l6144\_k10}
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,0.000233)(2,0.000475)(4,0.001249)(8,0.003)(16,0.00649)(32,0.010327)
                };
                \addlegendentry{TopK\_l1536\_k32}
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,0.000125)(2,0.000341)(4,0.000772)(8,0.001974)(16,0.005078)(32,0.008554)
                };
                \addlegendentry{TopK\_l3072\_k32}
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,0.000104)(2,0.000253)(4,0.000633)(8,0.001724)(16,0.004385)(32,0.007625)
                };
                \addlegendentry{TopK\_l6144\_k32}
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,0.000105)(2,0.000292)(4,0.000717)(8,0.001818)(16,0.004163)(32,0.007993)
                };
                \addlegendentry{TopK\_l1536\_k64}
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,8.8e-05)(2,0.000199)(4,0.000546)(8,0.001353)(16,0.00321)(32,0.006857)
                };
                \addlegendentry{TopK\_l3072\_k64}
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,4.1e-05)(2,0.00011)(4,0.000335)(8,0.000898)(16,0.002358)(32,0.005186)
                };
                \addlegendentry{TopK\_l6144\_k64}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={CLIP: TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,0.0167)(2,0.037)(4,0.0826)(8,0.1256)(16,0.1483)(32,0.1734)
                };
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,0.0133)(2,0.025)(4,0.0481)(8,0.0794)(16,0.0998)(32,0.1157)
                };
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,0.0098)(2,0.0178)(4,0.0362)(8,0.0637)(16,0.0835)(32,0.0994)
                };
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,0.0025)(2,0.0049)(4,0.0085)(8,0.0137)(16,0.0204)(32,0.0286)
                };
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,0.0022)(2,0.004)(4,0.0072)(8,0.0113)(16,0.0162)(32,0.0208)
                };
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,0.0014)(2,0.003)(4,0.0055)(8,0.0089)(16,0.0119)(32,0.0149)
                };
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,0.001)(2,0.0021)(4,0.0045)(8,0.0082)(16,0.0128)(32,0.0177)
                };
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,0.0006)(2,0.0013)(4,0.0028)(8,0.0054)(16,0.0088)(32,0.0126)
                };
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,0.0004)(2,0.0009)(4,0.0019)(8,0.0038)(16,0.0064)(32,0.0091)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={BLIP: TopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, dashed] coordinates {
                  (1,0.0095)(2,0.0176)(4,0.0325)(8,0.049)(16,0.0629)(32,0.079)
                };
                \addplot[color=blue, mark=square*, dashed] coordinates {
                  (1,0.0082)(2,0.0155)(4,0.0257)(8,0.0375)(16,0.0492)(32,0.0682)
                };
                \addplot[color=green!50!black, mark=square*, dashed] coordinates {
                  (1,0.0073)(2,0.0147)(4,0.0242)(8,0.0363)(16,0.0473)(32,0.0637)
                };
                \addplot[color=red, mark=triangle*, dashed] coordinates {
                  (1,0.0009)(2,0.0022)(4,0.0045)(8,0.0075)(16,0.0103)(32,0.0131)
                };
                \addplot[color=blue, mark=triangle*, dashed] coordinates {
                  (1,0.0006)(2,0.0016)(4,0.0034)(8,0.0058)(16,0.0085)(32,0.0114)
                };
                \addplot[color=green!50!black, mark=triangle*, dashed] coordinates {
                  (1,0.0006)(2,0.0013)(4,0.0028)(8,0.0049)(16,0.0075)(32,0.0102)
                };
                \addplot[color=red, mark=diamond*, dashed] coordinates {
                  (1,0.0003)(2,0.0008)(4,0.0018)(8,0.0036)(16,0.0062)(32,0.0091)
                };
                \addplot[color=blue, mark=diamond*, dashed] coordinates {
                  (1,0.0002)(2,0.0006)(4,0.0014)(8,0.0029)(16,0.0051)(32,0.0077)
                };
                \addplot[color=green!50!black, mark=diamond*, dashed] coordinates {
                  (1,0.0002)(2,0.0005)(4,0.0011)(8,0.0022)(16,0.0039)(32,0.0064)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}

    \vspace{0.4em}

    %% ===================== ROW 2: BatchTopKSAE =====================
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={DINO: BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 legend to name=legendBatch,
                 legend style={legend columns=3, font=\scriptsize, column sep=0.3cm},
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,0.000403)(2,0.000901)(4,0.002375)(8,0.006201)(16,0.009466)(32,0.012347)
                };
                \addlegendentry{BatchTopK\_l1536\_k10}
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,0.000202)(2,0.000591)(4,0.001589)(8,0.004415)(16,0.007571)(32,0.009646)
                };
                \addlegendentry{BatchTopK\_l3072\_k10}
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,0.000211)(2,0.000475)(4,0.001229)(8,0.003874)(16,0.006705)(32,0.00856)
                };
                \addlegendentry{BatchTopK\_l6144\_k10}
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,0.000192)(2,0.000525)(4,0.001351)(8,0.002871)(16,0.005996)(32,0.009888)
                };
                \addlegendentry{BatchTopK\_l1536\_k32}
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,0.000121)(2,0.000279)(4,0.000732)(8,0.001855)(16,0.004565)(32,0.008142)
                };
                \addlegendentry{BatchTopK\_l3072\_k32}
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,8.6e-05)(2,0.000205)(4,0.000524)(8,0.001334)(16,0.003604)(32,0.006881)
                };
                \addlegendentry{BatchTopK\_l6144\_k32}
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,0.000143)(2,0.000341)(4,0.000886)(8,0.002027)(16,0.004457)(32,0.008562)
                };
                \addlegendentry{BatchTopK\_l1536\_k64}
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,6.9e-05)(2,0.000179)(4,0.000459)(8,0.00104)(16,0.00298)(32,0.006405)
                };
                \addlegendentry{BatchTopK\_l3072\_k64}
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,4e-05)(2,0.000117)(4,0.000312)(8,0.000831)(16,0.002394)(32,0.005429)
                };
                \addlegendentry{BatchTopK\_l6144\_k64}
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={CLIP: BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,0.0169)(2,0.0336)(4,0.074)(8,0.106)(16,0.1276)(32,0.1408)
                };
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,0.0117)(2,0.0238)(4,0.0475)(8,0.0777)(16,0.097)(32,0.1103)
                };
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,0.01)(2,0.0223)(4,0.041)(8,0.0626)(16,0.0723)(32,0.0796)
                };
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,0.0023)(2,0.0047)(4,0.0085)(8,0.0132)(16,0.0199)(32,0.0284)
                };
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,0.0017)(2,0.0033)(4,0.006)(8,0.0096)(16,0.0145)(32,0.0208)
                };
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,0.0009)(2,0.002)(4,0.0042)(8,0.0066)(16,0.0098)(32,0.0137)
                };
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,0.0011)(2,0.0023)(4,0.0049)(8,0.0087)(16,0.013)(32,0.0183)
                };
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,0.0005)(2,0.0013)(4,0.0026)(8,0.0052)(16,0.0083)(32,0.0118)
                };
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,0.0003)(2,0.0007)(4,0.0016)(8,0.0032)(16,0.0055)(32,0.0082)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.33\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                 width=\textwidth,
                 height=0.85\textwidth,
                 xlabel={Number of deleted features (N)},
                 ylabel={Overall drop},
                 grid=both,
                 grid style={line width=.1pt, dashed, draw=gray!10},
                 major grid style={line width=.2pt,draw=gray!50},
                 xmode=log,
                 log basis x=2,
                 xtick={1,2,4,8,16,32},
                 xticklabels={$2^0$,$2^1$,$2^2$,$2^3$,$2^4$,$2^5$},
                 label style={font=\scriptsize},
                 tick label style={font=\scriptsize},
                 every axis title/.style={at={(0.5,1.0)}, above, font=\small},
                 title={BLIP: BatchTopKSAE},
                 mark size=1.2pt,
                 line width=0.6pt,
                 ]
                \addplot[color=red, mark=square*, solid] coordinates {
                  (1,0.0046)(2,0.0078)(4,0.0114)(8,0.015)(16,0.0194)(32,0.0235)
                };
                \addplot[color=blue, mark=square*, solid] coordinates {
                  (1,0.0034)(2,0.0059)(4,0.0085)(8,0.012)(16,0.0142)(32,0.0171)
                };
                \addplot[color=green!50!black, mark=square*, solid] coordinates {
                  (1,0.003)(2,0.0053)(4,0.0072)(8,0.0088)(16,0.0109)(32,0.0134)
                };
                \addplot[color=red, mark=triangle*, solid] coordinates {
                  (1,0.0004)(2,0.0009)(4,0.0021)(8,0.0039)(16,0.0058)(32,0.0077)
                };
                \addplot[color=blue, mark=triangle*, solid] coordinates {
                  (1,0.0002)(2,0.0007)(4,0.0018)(8,0.0031)(16,0.0044)(32,0.0058)
                };
                \addplot[color=green!50!black, mark=triangle*, solid] coordinates {
                  (1,0.0001)(2,0.0004)(4,0.0011)(8,0.002)(16,0.0032)(32,0.0043)
                };
                \addplot[color=red, mark=diamond*, solid] coordinates {
                  (1,0.0002)(2,0.0005)(4,0.0012)(8,0.0025)(16,0.005)(32,0.008)
                };
                \addplot[color=blue, mark=diamond*, solid] coordinates {
                  (1,0.0001)(2,0.0004)(4,0.0009)(8,0.0018)(16,0.0036)(32,0.0058)
                };
                \addplot[color=green!50!black, mark=diamond*, solid] coordinates {
                  (1,0.0001)(2,0.0002)(4,0.0005)(8,0.0011)(16,0.0023)(32,0.0042)
                };
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}

    \vspace{0.3em}
    \ref{legendTopK}\par\vspace{0.2em}
    \ref{legendBatch}

    \caption{Deletion curves showing overall drop as a function of number of deleted features (N). Top row: TopKSAE, bottom row: BatchTopKSAE. Columns: DINO, CLIP, BLIP.}
    \label{fig:deletion_curves_overall_per_metric}
\end{figure*}

==> TABS/correlation_analysis_tab.tex <==
\begin{table*}[]
    \centering
    \caption{Correlation analysis of TMS/MS-target drop across different models and N values. All correlations computed with corresponding p-values. Best results for each model marked in bold. Non-significant results (p-value > 0.05) in italics.}
    \label{table:correlation_analysis}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Model} & \multirow{2}{*}{N} & \multicolumn{2}{c|}{Target drop - TMS} & \multicolumn{2}{c|}{Target drop - MS}  \\ \cline{3-6}
                               &                    & Correlation & p-value & Correlation & p-value  \\ \hline
        \multirow{6}{*}{DINO}  & 1                  & 0.837 & 0.000015 & \textbf{0.878} & 0.000002  \\ \cline{2-6}
                               & 2                  & 0.878 & 0.000002 & \textbf{0.915} & 0.000000 \\ \cline{2-6}
                               & 4                  & 0.876 & 0.000002 & \textbf{0.893} & 0.000001  \\ \cline{2-6}
                               & 8                  & 0.843 & 0.000011 & \textbf{0.905} & 0.000000  \\ \cline{2-6}
                               & 16                 & 0.825 & 0.000026 & \textbf{0.917} & 0.000000  \\ \cline{2-6}
                               & 32                 & 0.868 & 0.000003 & \textbf{0.917} & 0.000000  \\ \hline
        \multirow{6}{*}{CLIP}  & 1                  & \textbf{0.783} & 0.000121 & 0.721 & 0.000728  \\ \cline{2-6}
                               & 2                  & \textbf{0.827} & 0.000023 & 0.707 & 0.001037  \\ \cline{2-6}
                               & 4                  & \textbf{0.864} & 0.000004 & 0.653 & 0.003286  \\ \cline{2-6}
                               & 8                  & \textbf{0.678} & 0.001985 & 0.534 & 0.022588  \\ \cline{2-6}
                               & 16                 & \textit{0.406} & \textit{0.094953} & \textit{0.257} & \textit{0.303309}  \\ \cline{2-6}
                               & 32                 & \textit{0.158} & \textit{0.531483} & \textit{-0.001} & \textit{0.996757}  \\ \hline
        \multirow{6}{*}{BLIP}  & 1                  & 0.719 & 0.000767 & \textbf{0.818} & 0.000033  \\ \cline{2-6}
                               & 2                  & 0.674 & 0.002166 & \textbf{0.785} & 0.000113  \\ \cline{2-6}
                               & 4                  & 0.622 & 0.005819 & \textbf{0.750} & 0.000335  \\ \cline{2-6}
                               & 8                  & 0.670 & 0.002360 & \textbf{0.771} & 0.000181  \\ \cline{2-6}
                               & 16                 & \textbf{0.697} & 0.001318 & 0.662 & 0.002791  \\ \cline{2-6}
                               & 32                 & \textbf{0.732} & 0.000558 & 0.577 & 0.012195  \\ \hline
    \end{tabular}
\end{table*}

==> TABS/stats_comparison_tab.tex <==
\begin{table*}[h]
    \centering
    \caption{Training metrics of SAE models across different feature extractors and configurations. $R^2$ denotes explained variance, $L_0$ denotes the average number of active latent dimensions, and CS denotes mean cosine similarity between input and reconstruction. Best $R^2$ and CS per feature extractor marked in bold.}
    \label{table:sae_training_metrics}
    \begin{tabular}{|c|c|c|cc|cc|cc|}
        \hline
        \multirow{2}{*}{Model} & \multirow{2}{*}{Exp.\ Factor} & \multirow{2}{*}{$K$} & \multicolumn{2}{c|}{$R^2$} & \multicolumn{2}{c|}{$L_0$} & \multicolumn{2}{c|}{CS} \\ \cline{4-9}
                               &                               &                      & BatchTopK & TopK & BatchTopK & TopK & BatchTopK & TopK \\ \hline
        \multirow{9}{*}{DINO} & \multirow{3}{*}{$\times$2} & 10 & 0.6652 & 0.6755 & 10.37 & 10 & 0.7959 & 0.8128 \\ \cline{3-9}
         &  & 32 & 0.7053 & 0.7053 & 33.18 & 32 & 0.8386 & 0.8339 \\ \cline{3-9}
         &  & 64 & 0.7244 & 0.7177 & 66.12 & 64 & 0.8473 & 0.8407 \\ \cline{2-9}
         & \multirow{3}{*}{$\times$4} & 10 & 0.6862 & 0.6962 & 10.37 & 10 & 0.8131 & 0.8253 \\ \cline{3-9}
         &  & 32 & 0.7336 & 0.7335 & 33.18 & 32 & 0.8465 & 0.8436 \\ \cline{3-9}
         &  & 64 & 0.7513 & 0.7390 & 66.35 & 64 & 0.8603 & 0.8523 \\ \cline{2-9}
         & \multirow{3}{*}{$\times$8} & 10 & 0.7030 & 0.7179 & 10.37 & 10 & 0.8182 & 0.8336 \\ \cline{3-9}
         &  & 32 & 0.7579 & 0.7472 & 33.18 & 32 & 0.8569 & 0.8528 \\ \cline{3-9}
         &  & 64 & \textbf{0.7688} & 0.7565 & 66.35 & 64 & \textbf{0.8637} & 0.8607 \\ \hline
        \multirow{9}{*}{CLIP} & \multirow{3}{*}{$\times$2} & 10 & 0.6728 & 0.7144 & 10.37 & 10 & 0.7618 & 0.8425 \\ \cline{3-9}
         &  & 32 & 0.8468 & 0.8481 & 33.18 & 32 & 0.9052 & 0.9167 \\ \cline{3-9}
         &  & 64 & 0.8904 & 0.8889 & 66.35 & 64 & \textbf{0.9435} & 0.9389 \\ \cline{2-9}
         & \multirow{3}{*}{$\times$4} & 10 & 0.6686 & 0.7096 & 10.37 & 10 & 0.7432 & 0.8407 \\ \cline{3-9}
         &  & 32 & 0.8485 & 0.8549 & 33.18 & 32 & 0.8886 & 0.9199 \\ \cline{3-9}
         &  & 64 & 0.8922 & 0.8952 & 66.35 & 64 & 0.9410 & 0.9412 \\ \cline{2-9}
         & \multirow{3}{*}{$\times$8} & 10 & 0.6852 & 0.7046 & 10.37 & 10 & 0.7519 & 0.8356 \\ \cline{3-9}
         &  & 32 & 0.8566 & 0.8557 & 33.18 & 32 & 0.8828 & 0.9191 \\ \cline{3-9}
         &  & 64 & 0.8979 & \textbf{0.8993} & 66.35 & 64 & 0.9375 & 0.9413 \\ \hline
        \multirow{9}{*}{BLIP} & \multirow{3}{*}{$\times$2} & 10 & 0.6173 & 0.6498 & 10.37 & 10 & 0.6777 & 0.8054 \\ \cline{3-9}
         &  & 32 & 0.7977 & 0.7923 & 33.18 & 32 & 0.8798 & 0.8884 \\ \cline{3-9}
         &  & 64 & 0.8289 & 0.8099 & 65.24 & 64 & 0.9055 & 0.9019 \\ \cline{2-9}
         & \multirow{3}{*}{$\times$4} & 10 & 0.6223 & 0.6655 & 10.37 & 10 & 0.6750 & 0.8161 \\ \cline{3-9}
         &  & 32 & 0.8048 & 0.8009 & 33.18 & 32 & 0.8707 & 0.8932 \\ \cline{3-9}
         &  & 64 & \textbf{0.8340} & 0.8259 & 65.70 & 64 & \textbf{0.9106} & 0.9065 \\ \cline{2-9}
         & \multirow{3}{*}{$\times$8} & 10 & 0.6372 & 0.6687 & 10.37 & 10 & 0.6636 & 0.8152 \\ \cline{3-9}
         &  & 32 & 0.8099 & 0.8057 & 33.18 & 32 & 0.8666 & 0.8939 \\ \cline{3-9}
         &  & 64 & 0.8283 & 0.7925 & 65.47 & 64 & \textbf{0.9106} & 0.8992 \\ \hline
    \end{tabular}
\end{table*}

